In-the-loop Hyper-Parameter Optimization for LLM-Based Automated Design of Heuristics

Large Language Models (LLMs) have shown great potential in automatically generating and optimizing (meta)heuristics, making them valuable tools in heuristic optimization tasks. However, LLMs are generally inefficient when it comes to fine-tuning hyper-parameters of the generated algorithms, often requiring excessive queries that lead to high computational and financial costs. This paper presents a novel hybrid approach, LLaMEA-HPO, which integrates the open source LLaMEA (Large Language Model Evolutionary Algorithm) framework with a Hyper-Parameter Optimization (HPO) procedure in the loop. By offloading hyper-parameter tuning to an HPO procedure, the LLaMEA-HPO framework allows the LLM to focus on generating novel algorithmic structures, reducing the number of required LLM queries and improving the overall efficiency of the optimization process. We empirically validate the proposed hybrid framework on benchmark problems, including Online Bin Packing, Black-Box Optimization, and the Traveling Salesperson Problem. Our results demonstrate that LLaMEA-HPO achieves superior or comparable performance compared to existing LLM-driven frameworks while significantly reducing computational costs. This work highlights the importance of separating algorithmic innovation and structural code search from parameter tuning in LLM-driven code optimization and offers a scalable approach to improve the efficiency and effectiveness of LLM-based code generation.

==> coverletter.tex <==
Dear Dr. Hemberg, Dr. O'Reilly, and Dr. Wilson,

I am pleased to submit our manuscript titled "In-the-loop Hyper-Parameter Optimization for LLM-Based Automated Design of Heuristics" for consideration in the special issue of ACM Transactions on Evolutionary Learning and Optimization on Integrating Evolutionary Algorithms and Large Language Models. This paper presents a novel hybrid framework, LLaMEA-HPO, that integrates the Large Language Model Evolutionary Algorithm (LLaMEA) with Hyper-Parameter Optimization (HPO) to enhance the efficiency of LLM-driven code generation in optimization tasks.

Our work directly addresses the themes of this special issue, specifically focusing on the combination of evolutionary algorithms and LLMs for hyper-parameter tuning and algorithm generation. The paper presents empirical results on benchmark problems, including Online Bin Packing, Black-Box Optimization, and the Traveling Salesperson Problem, demonstrating that LLaMEA-HPO significantly reduces the number of LLM queries required while maintaining high solution quality. This work advances current research by separating algorithmic creativity from parameter tuning, a key challenge in LLM-driven optimization tasks.

We believe our contribution is particularly relevant to topics such as:

LLM-assisted evolution and its impact on algorithmic creativity.
The integration of LLMs with evolutionary operators to enhance scalability.
Novel hybrid approaches that combine HPO and LLMs for metaheuristic optimization.
As per the submission guidelines, we confirm that this manuscript has not been submitted for publication elsewhere.

We appreciate your consideration of our submission and look forward to your feedback. Please do not hesitate to contact us if any additional information is required.

Sincerely,

Dr. Niki van Stein
LIACS, Leiden University

